Learning to Scale Logits for Temperature-Conditional GFlowNets

GFlowNets are probabilistic models that sequentially generate compositional structures through a stochastic policy. Among GFlowNets, temperature-conditional GFlowNets can introduce temperature-based controllability for exploration and exploitation. We propose \textit{Logit-scaling GFlowNets} (Logit-GFN), a novel architectural design that greatly accelerates the training of temperature-conditional GFlowNets. It is based on the idea that previously proposed approaches introduced numerical challenges in the deep network training, since different temperatures may give rise to very different gradient profiles as well as magnitudes of the policy's logits. We find that the challenge is greatly reduced if a learned function of the temperature is used to scale the policy's logits directly. Also, using Logit-GFN, GFlowNets can be improved by having better generalization capabilities in offline learning and mode discovery capabilities in online learning, which is empirically verified in various biological and chemical tasks. Our code is available at \url{https://github.com/dbsxodud-11/logit-gfn}

==> tables/table_qm9.tex <==
\begin{table*}[h]
\centering
\caption{{Perfomance evaluation on various metrics on QM9 task \textcolor{red}{(on going)}.}}\label{tab:orignal_table}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{llllllll}
\toprule
 Method&Type&Num. Modes & 75th percentile& 50th percentile&TopK score &Diversity \\
\midrule

SQL \cite{haarnoja2017reinforcement}
&
RL
&
25 $\pm$ 5


&

&

&

&

\\


PPO \cite{schulman2017proximal}
&
RL
&

4 $\pm$ 1

&

&

&

&

\\
\midrule

MARS$^\dagger$ \cite{xie2020mars}
&
MCMC
&
141 $\pm$ 44
&

&
&

&



\\
\midrule
DB \cite{bengio2023jmlr}
&
GFN
&
130
&

&

&

&




\\
TB \cite{malkin2022trajectory}
&
GFN
&
247 $\pm$ 26
&

&

&

&



\\
Sub-TB \cite{madan2023learning}
&
GFN
&
180
&

&

&


&


\\
GTB \cite{shen2023towards}
&
GFN
&
222
&

&

&
&




\\
Temp-GFN (\textit{logit})
&
GFN
&
\textbf{327} $\pm$ 103
&

&
2.11 $\pm$ 0.21 
&

&
\\
Temp-GFN (\textit{layer})
&
GFN
&
\textbf{327} $\pm$ 103
&

&
2.11 $\pm$ 0.21 
&

&



\\


\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table*}

==> tables/table_tfbind.tex <==
\begin{table*}[h]
\centering
\caption{{Perfomance evaluation on various metrics on TFbind8 task \textcolor{red}{(on going)}.}}\label{tab:orignal_table}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{llllllll}
\toprule
 Method&Type&Num. Modes & 75th percentile& 50th percentile&TopK score &Diversity \\
\midrule

A2C 
&
RL
&

&

&

&

&

\\

SQL \cite{haarnoja2017reinforcement}
&
RL
&

&

&

&

&

\\


PPO \cite{schulman2017proximal}
&
RL
&


&

&

&

&

\\
\midrule

MARS$^\dagger$ \cite{xie2020mars}
&
MCMC
&

&

&
&

&



\\
% \midrule
% DB \cite{bengio2023jmlr}
% &
% GFN
% &

% &

% &

% &

% &




% \\
TB \cite{malkin2022trajectory}
&
GFN
&

&

&

&

&



% \\
% Sub-TB \cite{madan2023learning}
% &
% GFN
% &

% &

% &

% &


% &


% \\
% GTB \cite{shen2023towards}
% &
% GFN
% &

% &

% &

% &
% &




\\
Temp-GFN (\textit{logit})
&
GFN
&
\textbf{327} $\pm$ 103
&

&
2.11 $\pm$ 0.21 
&

&
\\
Temp-GFN (\textit{layer})
&
GFN
&
\textbf{327} $\pm$ 103
&

&
2.11 $\pm$ 0.21 
&

&

\\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table*}
